nnU-Net Revisited: A Call for Rigorous Validation in 3D Medical Image Segmentation

The release of nnU-Net marked a paradigm shift in 3D medical image segmentation, demonstrating that a properly configured U-Net architecture could still achieve state-of-the-art results. Despite this, the pursuit of novel architectures, and the respective claims of superior performance over the U-Net baseline, continued. In this study, we demonstrate that many of these recent claims fail to hold up when scrutinized for common validation shortcomings, such as the use of inadequate baselines, insufficient datasets, and neglected computational resources. By meticulously avoiding these pitfalls, we conduct a thorough and comprehensive benchmarking of current segmentation methods including CNN-based, Transformer-based, and Mamba-based approaches. In contrast to current beliefs, we find that the recipe for state-of-the-art performance is 1) employing CNN-based U-Net models, including ResNet and ConvNeXt variants, 2) using the nnU-Net framework, and 3) scaling models to modern hardware resources. These results indicate an ongoing innovation bias towards novel architectures in the field and underscore the need for more stringent validation standards in the quest for scientific progress.

==> notes.tex <==
%In one instance, nnU-Net's results were incorrectly cited \cite{unetr}, with these erroneous figures being further propagated in subsequent research \cite{jiang2022self}.

%Unfortunately this problem can be further exacerbated by the authors of the architectures serving as baseline not providing explicit instructions on how to properly set-up their architectures for new datasets (see P6). 

%My take on this:
%- even if leaderbords exist, there are no standardized rules for what should be submitted, leading to researchers submitting a heterogeneous landscape of single models, small and large ensembles, with and without test time augmentations and (architecture independent) postprocessing techniques. Submitting to test sets is important (to show that your method can hold its ground in a highly competitive setting) but it ultimately does not allow us to make methodological conclusions
%- this causes studies to prefer reporting on a custom train/test split so that they can compare their method versus the baselines in a controlled setting. Such custom splits have typically unreasonably small test sets, causing substantial instability in the results and making small gains questionable
%- a better approach would be to run a 5-fold cross-validation with a rotating val set (though this potentially allows methods to overfit to development datasets)
%- best would be to have a development pool and an independent test pool of datasets. Evaluate proposed method vs baselines on a cross-validation on the test pool.
%- (+ what you said about subset of classes)


%While utilizing public test set leaderboards is often the preferred method for reporting results, the practice of making multiple submissions to the same leaderboard can inadvertently result in overfitting, particularly with smaller test sets. Additionally, many widely-used benchmark datasets lack associated leaderboards, leading the research community to adopt the practice of reporting results through 5-fold cross-validation on the training set. However, some studies deviate by reporting results based on a single, custom train-test split. This approach makes the results highly dependent on the specific split limiting their comparability \cite{wu2023d,xu2023levit,zhou2021nnformer}. Another concerning practice involves reporting results on a selected subset of classes from datasets such as BTCV without valid justification for excluding others, further undermining the integrity of results \cite{zhou2021nnformer,chen2021transunet,cao2022swin,wu2023d,xu2023levit}. 
%Actively ignoring the presence of public test set (Single 80-15-5 split, on MSD001\_BrainTumour which has an active leaderboard as in nnFormer). BTCV: 

    

